EdinburghNLP at WNUT-2020 Task 2: Leveraging Transformers with Generalized Augmentation for Identifying Informativeness in COVID-19 Tweets

Twitter and, in general, social media has become an indispensable communication channel in times of emergency. The ubiquitousness of smartphone gadgets enables people to declare an emergency observed in real-time. As a result, more agencies are interested in programmatically monitoring Twitter (disaster relief organizations and news agencies). Therefore, recognizing the informativeness of a Tweet can help filter noise from the large volumes of Tweets. In this paper, we present our submission for WNUT-2020 Task 2: Identification of informative COVID-19 English Tweets. Our most successful model is an ensemble of transformers, including RoBERTa, XLNet, and BERTweet trained in a Semi-Supervised Learning (SSL) setting. The proposed system achieves an F1 score of 0.9011 on the test set (ranking 7th on the leaderboard) and shows significant gains in performance compared to a baseline system using FastText embeddings.

==> tables/tweet_example.tex <==
\begin{table}[h]
  \centering
    \begin{tabular}{ | c | c |}
      \hline
      \thead{\textbf{Text}} & \thead{\textbf{Label}}\\
      \hline
      \makecell{\small{1) Some thoughts on China’s 1Q macro}\\\small{numbers. China’s economy was the first to}\\\small{suffer the consequences of fighting the novel}\\\small{coronavirus and is the first on the road to}\\\small{recovery. After an initial cover-up and more}\\\small{than 3,000 deaths, China appears to have}\\\small{brought COVID-19}} & 0\\
      \hline
    \end{tabular}
\caption{\label{table:Tweet} A hard to classify tweet.}
\end{table}
